CHANG-ES XXVI: Insights into cosmic-ray transport from radio halos in edge-on galaxies

Galactic winds play a key role in regulating the evolution of galaxies over cosmic time. In recent years, the role of cosmic rays (CR) in the formation of the galactic wind has increasingly gained attention. Therefore, we use radio continuum data to analyse the cosmic ray transport in edge-on galaxies. Data from the LOFAR Two-metre Sky Survey (LoTSS) data release 2 at 144 MHz (HBA) and reprocessed VLA data at 1.6 GHz (L-band) from the Continuum Halos in Nearby Galaxies - an EVLA Survey (CHANG-ES) enable us to increase the extent of the analysed radio continuum profile significantly (up to a factor of 2) compared to previous studies. We compute thermal emission maps using a mixture approach of H-alpha and near infrared data, which is then subtracted to yield radio synchrotron emission maps. Then we compile non-thermal spectral index maps and compute intensity profiles using a box integration approach. Lastly, we perform 1D cosmic ray transport modelling. The non-thermal spectral index maps show evidence that the LoTSS maps are affected by thermal absorption, in star forming regions. The scale height analysis reveals that most of the galaxies are equally well fitted with an one-component instead of a twocomponent exponential profile. We find a bi-modality within our sample. While NGC 3432 and NGC 4013 have similar scale heights in the L-band and HBA, the low-frequency scale heights of NGC 891, NGC 4157, and NGC 4631 exceed their high-frequency counterpart significantly. The 1D CR transport modelling shows agreement of the predicted magnetic field strength and the magnetic field strength estimates of equipartition measurements. Additionally we find an increasing difference of wind velocities (with increasing height over the galactic disk) between central and outer regions of the analysed galaxies.

==> CHANG-ES CR Transport MStein/figures/total_intensity/tab_fit_params.tex <==
\begin{tabular}{lrlllllllr}
\toprule
N3432 & 1500 & one\_fo & LR & 0.32$\pm$0.04 &   1.16$\pm$0.09 &             - &             - &              - &  3.72 \\
N3432 &  144 & one\_fo & LR &   7.5$\pm$2.3 &   0.28$\pm$0.07 &             - &             - &              - &  2.41 \\
N3432 & 1500 &     one & UR & 2.20$\pm$0.20 &   0.45$\pm$0.03 &             - &             - &  0.54$\pm$0.07 &  4.27 \\
N3432 &  144 &     one & UR &     31$\pm$21 &   0.13$\pm$0.09 &             - &             - &  0.72$\pm$0.06 &  1.39 \\
N3432 & 1500 & one\_fo & LM & 4.68$\pm$0.27 & 0.940$\pm$0.028 &             - &             - &              - &  5.23 \\
N3432 &  144 & one\_fo & LM &  16.7$\pm$1.3 &   1.01$\pm$0.04 &             - &             - &              - &  1.11 \\
N3432 & 1500 & one\_fo & UM & 4.43$\pm$0.21 & 0.789$\pm$0.019 &             - &             - &              - & 10.07 \\
N3432 &  144 & one\_fo & UM &  16.7$\pm$1.2 &   0.87$\pm$0.03 &             - &             - &              - &  2.26 \\
N3432 & 1500 & one\_fo & LL & 2.47$\pm$0.29 &   0.91$\pm$0.05 &             - &             - &              - &  1.44 \\
N3432 &  144 & one\_fo & LL &   8.0$\pm$1.0 &   1.14$\pm$0.07 &             - &             - &              - &  1.77 \\
N3432 & 1500 & one\_fo & UL & 1.55$\pm$0.16 &   0.91$\pm$0.05 &             - &             - &              - &  1.97 \\
N3432 &  144 & one\_fo & UL &   6.2$\pm$0.8 &   1.03$\pm$0.07 &             - &             - &              - &  1.50 \\
N4013 & 1500 & one\_fo & LR & 2.09$\pm$0.19 & 0.607$\pm$0.026 &             - &             - &              - &  1.42 \\
N4013 &  144 & one\_fo & LR &   9.6$\pm$1.0 &   0.75$\pm$0.04 &             - &             - &              - &  0.55 \\
N4013 & 1500 & one\_fo & UR & 2.28$\pm$0.22 &   0.74$\pm$0.04 &             - &             - &              - &  0.96 \\
N4013 &  144 & one\_fo & UR &   9.1$\pm$1.0 &   0.87$\pm$0.04 &             - &             - &              - &  7.19 \\
N4013 & 1500 & one\_fo & LM &   4.3$\pm$0.4 & 0.549$\pm$0.025 &             - &             - &              - & 12.45 \\
N4013 &  144 & one\_fo & LM &  20.6$\pm$2.1 & 0.639$\pm$0.026 &             - &             - &              - &  3.15 \\
N4013 & 1500 & one\_fo & UM &   9.1$\pm$0.8 & 0.483$\pm$0.018 &             - &             - &              - &  3.54 \\
N4013 &  144 & one\_fo & UM &  30.9$\pm$2.8 & 0.642$\pm$0.022 &             - &             - &              - &  4.04 \\
N4013 & 1500 & one\_fo & LL & 2.45$\pm$0.18 & 0.670$\pm$0.030 &             - &             - &              - &  2.89 \\
N4013 &  144 & one\_fo & LL &  10.0$\pm$1.0 &   0.74$\pm$0.04 &             - &             - &              - &  1.41 \\
N4013 & 1500 & one\_fo & UL & 3.38$\pm$0.22 & 0.582$\pm$0.020 &             - &             - &              - &  2.52 \\
N4013 &  144 & two\_fo & UL &  12.8$\pm$1.7 &   0.64$\pm$0.13 &   0.6$\pm$0.6 &       5$\pm$5 &              - &  0.73 \\
N4157 & 1500 & one\_fo & LR &   3.2$\pm$0.4 &   1.32$\pm$0.07 &             - &             - &              - &  0.68 \\
N4157 &  144 &     one & LR &  15.7$\pm$2.3 &   1.25$\pm$0.07 &             - &             - &  0.55$\pm$0.26 &  5.26 \\
N4157 & 1500 & one\_fo & UR &   3.7$\pm$0.6 &   0.96$\pm$0.06 &             - &             - &              - &  0.17 \\
N4157 &  144 & one\_fo & UR &   6.9$\pm$1.2 &   2.31$\pm$0.19 &             - &             - &              - &  6.10 \\
N4157 & 1500 & one\_fo & LM &  13.6$\pm$0.6 & 1.121$\pm$0.021 &             - &             - &              - &  4.79 \\
N4157 &  144 & two\_fo & LM &      66$\pm$7 &   0.88$\pm$0.11 &   8.6$\pm$2.0 &   3.5$\pm$0.3 &              - &  2.34 \\
N4157 & 1500 & two\_fo & UM &       8$\pm$7 &     0.7$\pm$0.4 &       9$\pm$8 & 1.25$\pm$0.20 &              - &  0.65 \\
N4157 &  144 &     two & UM &      64$\pm$5 &   1.21$\pm$0.10 &   1.3$\pm$0.6 &      10$\pm$5 &  0.24$\pm$0.17 &  2.88 \\
N4157 & 1500 & one\_fo & LL &   2.6$\pm$0.4 &   0.96$\pm$0.08 &             - &             - &              - &  0.03 \\
N4157 &  144 & one\_fo & LL &   5.0$\pm$0.8 &   2.63$\pm$0.19 &             - &             - &              - &  4.17 \\
N4157 & 1500 & one\_fo & UL &   2.4$\pm$0.3 &   1.45$\pm$0.07 &             - &             - &              - &  2.24 \\
N4157 &  144 & one\_fo & UL &  10.0$\pm$1.1 &   2.59$\pm$0.13 &             - &             - &              - &  0.40 \\
N4631 & 1500 & one\_fo & LR &   6.8$\pm$0.4 & 1.053$\pm$0.029 &             - &             - &              - &  1.11 \\
N4631 &  144 & one\_fo & LR &  19.4$\pm$1.1 &   1.89$\pm$0.05 &             - &             - &              - &  0.74 \\
N4631 & 1500 &     two & UR &  10.5$\pm$2.8 &   0.52$\pm$0.16 & 0.89$\pm$0.22 &   2.6$\pm$0.3 &   -0.6$\pm$0.4 &  0.39 \\
N4631 &  144 & two\_fo & UR &  11.6$\pm$1.3 &   1.44$\pm$0.27 &   2.7$\pm$1.2 &   4.5$\pm$0.8 &              - &  1.07 \\
N4631 & 1500 &     two & LM &     42$\pm$16 &   0.59$\pm$0.10 &   6.3$\pm$1.2 & 1.80$\pm$0.07 &   -0.7$\pm$0.4 &  1.88 \\
N4631 &  144 & two\_fo & LM &  37.0$\pm$2.9 &   1.46$\pm$0.12 &   3.0$\pm$1.0 &   5.3$\pm$0.7 &              - &  5.03 \\
N4631 & 1500 &     two & UM &     45$\pm$10 &   0.39$\pm$0.11 &   5.0$\pm$0.6 & 2.01$\pm$0.05 & -0.44$\pm$0.27 &  1.68 \\
N4631 &  144 & one\_fo & UM &  19.1$\pm$0.8 &   2.90$\pm$0.05 &             - &             - &              - &  4.45 \\
N4631 & 1500 & one\_fo & LL & 2.00$\pm$0.14 &   1.93$\pm$0.06 &             - &             - &              - &  1.12 \\
N4631 &  144 & one\_fo & LL &   8.6$\pm$0.5 &   2.84$\pm$0.07 &             - &             - &              - &  0.86 \\
N4631 & 1500 & one\_fo & UL & 1.15$\pm$0.09 &   2.15$\pm$0.09 &             - &             - &              - &  1.07 \\
N4631 &  144 & one\_fo & UL &   6.1$\pm$0.3 &   3.71$\pm$0.10 &             - &             - &              - &  0.75 \\
 N891 & 1500 & one\_fo & LR &   4.3$\pm$0.3 &   1.09$\pm$0.04 &             - &             - &              - &  2.55 \\
 N891 &  144 & one\_fo & LR &  15.2$\pm$1.0 &   1.85$\pm$0.04 &             - &             - &              - &  4.02 \\
 N891 & 1500 & one\_fo & UR &   4.5$\pm$0.3 &   1.35$\pm$0.04 &             - &             - &              - &  3.50 \\
 N891 &  144 & two\_fo & UR &      32$\pm$5 &   0.77$\pm$0.15 &   6.7$\pm$1.4 & 3.04$\pm$0.26 &              - &  3.41 \\
 N891 & 1500 & one\_fo & LM &  17.2$\pm$0.8 & 0.822$\pm$0.016 &             - &             - &              - &  7.41 \\
 N891 &  144 &     two & LM &   188$\pm$113 &   0.87$\pm$0.08 &   5.8$\pm$2.1 &   2.9$\pm$0.4 &   -1.0$\pm$0.7 &  1.01 \\
 N891 & 1500 & one\_fo & UM &  16.9$\pm$0.6 & 1.176$\pm$0.014 &             - &             - &              - &  5.88 \\
 N891 &  144 &     two & UM &    111$\pm$18 &   1.05$\pm$0.10 &   6.6$\pm$2.3 &   3.6$\pm$0.5 & -0.33$\pm$0.27 &  0.50 \\
 N891 & 1500 & one\_fo & LL &   7.4$\pm$0.6 &   1.05$\pm$0.03 &             - &             - &              - &  1.21 \\
 N891 &  144 & two\_fo & LL &     43$\pm$22 &   0.37$\pm$0.21 &  13.9$\pm$1.6 & 2.18$\pm$0.08 &              - &  1.22 \\
 N891 & 1500 & one\_fo & UL &   6.9$\pm$0.6 &   1.07$\pm$0.04 &             - &             - &              - &  1.05 \\
 N891 &  144 & one\_fo & UL &  25.4$\pm$1.9 &   1.67$\pm$0.05 &             - &             - &              - &  1.05 \\
\bottomrule
\end{tabular}


==> CHANG-ES CR Transport MStein/si_fig.tex <==
\begin{figure*}
\centering
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{figures/si_maps/NGC891_Non-Thermal_SI.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{figures/si_maps/NGC3432_Non-Thermal_SI.png}
\end{subfigure}
\\
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/si_maps/NGC4013_Non-Thermal_SI.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/si_maps/NGC4157_Non-Thermal_SI.png}
\end{subfigure}
\\
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/si_maps/NGC4631_Non-Thermal_SI.png}
\end{subfigure}
\caption{Non-thermal spectral index (L-band corrected for thermal emission \& uncorrected HBA) maps. We use a custom colormap, where a flat SI is coloured blue to plum and a steep SI orange to yellow. The beam is displayed in the bottom right corner of each map as black circle.}
\label{fig:si_maps}
\end{figure*}

%%TW: Change SI in the figures to alpha, and in the caption to spectral index

==> CHANG-ES CR Transport MStein/tab_basic_info.tex <==
\begin{table*}
\caption{Fundamental information about the galaxies analysed in this work: Celestial coordinates at epoch J2000.0\tablefootmark{a}, morphological type\tablefootmark{b}, position angle\tablefootmark{b}, inclination\tablefootmark{c}, distance\tablefootmark{d}, diameter (based on $22\,\upmu$m WISE map)\tablefootmark{d}, rotational velocity\tablefootmark{c},  total baryon mass\tablefootmark{e}. }
\label{tab:basic_info}
\centering
\begin{tabular}{lrrrrrrrrr}
     \hline\hline
     Galaxy & RA & Dec & Morph. Type  & PA & Incl. & Distance & Diam. & $\varv_{\mathrm{rot}}$ & M\textsubscript{baryonic}\\
            &  [H:M:S] &  [D:M:S] &  & [$^\circ$] & [$^\circ$] & [Mpc] & [kpc] & [km\,s\textsuperscript{-1}] & [M$_\odot$]$\cdot$10\textsuperscript{10}\\
    \hline
    NGC~891     & 02h22m33.41s  & +42d20m56.9s  & Sb    & 22.0 & 90.0 & 9.1 & 25.1 & 212 & 8.63\\
    NGC~3432    & 10h52m31.13s  & +36d37m07.6s  & SBm   & 33.0 & 85.0 & 9.4 & 9.96 & 110 & 0.86\\
    NGC~4013    & 11h58m31.380s & +43d56m47.70s & SABb  & 58.6 & 88.0 & 16 & 16.1 & 182 &  4.99\\
    NGC~4157    & 12h11m04.37s  & +50d29m04.8s  & SABb  & 64.7 & 83.0 & 15.6 &  16.6 & 189 & 5.75 \\
    NGC~4631    & 12h42m08.01s  & +32d32m29.4s  & SBcd  & 85.7 & 85.0 &  7.4 & 23.4 & 139 & 1.93\\
    \hline
\end{tabular}

\tablefoot{\\
\tablefoottext{a}{Taken from the NASA NED (\url{https://ned.ipac.caltech.edu/}).\\}
\tablefoottext{b}{Taken from the HyperLeda Database (\url{http://leda.univ-lyon1.fr/}).\\}
\tablefoottext{c}{Taken from \citet{2022arXiv220400635H}\\}
\tablefoottext{d}{Taken from \citet{2015AJ....150...81W}\\}
\tablefoottext{e}{Taken from \citet{2016MNRAS.456.1723L}}
}
\end{table*}

==> CHANG-ES CR Transport MStein/tab_box_setup.tex <==
\begin{table*}
\centering
\caption{Box widths (W) used for box integration, radio beam FWHM converted to physical scales, assumed flux tube radius (R\textsubscript{0}) used for cosmic ray transport modelling for each galaxy; SFR, SFR surface density, and average equipartition magnetic field strength in the galactic disk for individual stripes; gravitational pull for central and outer stripes (as we assume the gravitational potential to be symmetric, there is no distinction for left and right stripes).}             % title of Table
\label{tab:box_setup}      % is used to refer this table in the text
%\centering                          % used for centering table
\begin{tabular}{l r r r | r r r | r r r | r r r | r r}        % centered columns (4 columns)
    \hline\hline                 % inserts double horizontal lines
    Galaxy  & W         & Beam  & R\textsubscript{0}& \multicolumn{3}{c}{SFR}                           & \multicolumn{3}{|c}{$\Sigma$\textsubscript{SFR}} & \multicolumn{3}{|c}{B-Field Strength} & \multicolumn{2}{|c}{Gravitational Pull}\\
            &[\arcsec]  &[kpc]  & [kpc]             &\multicolumn{3}{|c}{[M\textsubscript{\(\odot\)}\,yr\textsuperscript{-1}]} & \multicolumn{3}{|c}{[M\textsubscript{\(\odot\)}\,yr\textsuperscript{-1}\,kpc\textsuperscript{-2}]$\cdot10^{-3}$}& \multicolumn{3}{|c}{[\textmu G]} & \multicolumn{2}{|c}{[N]$\cdot10^{-10}$}\\% table heading \\
            &           &       &                   & left & middle & right & left & middle & right & left & middle & right & middle & outer\\ 

    \hline                        % inserts single horizontal line
    NGC~891  & 177   & 0.88 & 7.8    & 0.5 & 1.0 & 0.4   & 3.9 & 5.6 & 2.8   & 9.2 & 13.1 & 9.0 & 3.7 & 0.6\\       % inserting body of the table
    NGC~3432 & 102   & 0.91 & 4.6      & 0.2 & 0.3 & 0.1   & 3.7 & 4.2 & 1.1   & 8.6 & 10.2 & 6.7 & 1.6 & 0.3\\
    NGC~4013 & 63    & 1.36 & 4.3      & 0.2 & 0.3 & 0.1   & 4.6 & 5.6 & 3.8   & 7.5 &  9.1 & 7.3 & 5.0 & 0.8\\  
    NGC~4157 & 120   & 1.51 & 9.0   & 0.2 & 1.3 & 0.2   & 1.3 & 5.5 & 1.2   & 8.1 & 13.1 & 7.4 & 2.5 & 0.4\\ 
    NGC~4631 & 266   & 0.72 & 9.6    & 0.3 & 1.6 & 0.5   & 1.8 & 6.1 & 2.8   & 7.5 & 11.7 & 8.9 & 1.3 & 0.2\\ 
\hline                                   %inserts single line
\end{tabular}\\
\end{table*}

==> CHANG-ES CR Transport MStein/tab_fit_params.tex <==
\begingroup
\renewcommand{\arraystretch}{0.8} % Default value: 1
\begin{tabular}{lrlllllllr}
\hline
\hline
Galaxy & $\nu$ & Model & ID & $w_0$ & $z_0$ & $w_1$ & $z_1$ & $Z_0$ & $\chi^2_\nu$\\
 & [MHz] & & & [\textmu Jy\,Beam\textsuperscript{-1}] & [kpc] & [\textmu Jy\,Beam\textsuperscript{-1}] & [kpc] & [kpc] &\\
\toprule
N~3432 & 1500 & one\_fo & LR & 0.32$\pm$0.04 &   1.16$\pm$0.09 &             - &             - &              - &  3.72 \\
N~3432 &  144 & one\_fo & LR &   7.5$\pm$2.3 &   0.28$\pm$0.07 &             - &             - &              - &  2.41 \\
N~3432 & 1500 &     one & UR & 2.20$\pm$0.20 &   0.45$\pm$0.03 &             - &             - &  0.54$\pm$0.07 &  4.27 \\
N~3432 &  144 &     one & UR &     31$\pm$21 &   0.13$\pm$0.09 &             - &             - &  0.72$\pm$0.06 &  1.39 \\
N~3432 & 1500 & one\_fo & LM & 4.68$\pm$0.27 & 0.940$\pm$0.028 &             - &             - &              - &  5.23 \\
N~3432 &  144 & one\_fo & LM &  16.7$\pm$1.3 &   1.01$\pm$0.04 &             - &             - &              - &  1.11 \\
N~3432 & 1500 & one\_fo & UM & 4.43$\pm$0.21 & 0.789$\pm$0.019 &             - &             - &              - & 10.07 \\
N~3432 &  144 & one\_fo & UM &  16.7$\pm$1.2 &   0.87$\pm$0.03 &             - &             - &              - &  2.26 \\
N~3432 & 1500 & one\_fo & LL & 2.47$\pm$0.29 &   0.91$\pm$0.05 &             - &             - &              - &  1.44 \\
N~3432 &  144 & one\_fo & LL &   8.0$\pm$1.0 &   1.14$\pm$0.07 &             - &             - &              - &  1.77 \\
N~3432 & 1500 & one\_fo & UL & 1.55$\pm$0.16 &   0.91$\pm$0.05 &             - &             - &              - &  1.97 \\
N~3432 &  144 & one\_fo & UL &   6.2$\pm$0.8 &   1.03$\pm$0.07 &             - &             - &              - &  1.50 \\
N~4013 & 1500 & one\_fo & LR & 2.09$\pm$0.20 & 0.607$\pm$0.027 &             - &             - &              - &  1.77 \\
N~4013 &  144 & one\_fo & LR &   9.6$\pm$1.0 &   0.75$\pm$0.04 &             - &             - &              - &  0.55 \\
N~4013 & 1500 & one\_fo & UR & 2.32$\pm$0.22 &   0.73$\pm$0.04 &             - &             - &              - &  0.83 \\
N~4013 &  144 & one\_fo & UR &  12.4$\pm$1.4 &   0.69$\pm$0.04 &             - &             - &              - &  0.12 \\
N~4013 & 1500 & one\_fo & LM &   4.7$\pm$0.5 & 0.526$\pm$0.025 &             - &             - &              - &  8.92 \\
N~4013 &  144 & one\_fo & LM &  20.6$\pm$2.1 & 0.639$\pm$0.026 &             - &             - &              - &  3.15 \\
N~4013 & 1500 & one\_fo & UM &   9.4$\pm$0.9 & 0.476$\pm$0.018 &             - &             - &              - &  0.97 \\
N~4013 &  144 & one\_fo & UM &      33$\pm$3 & 0.614$\pm$0.023 &             - &             - &              - &  0.30 \\
N~4013 & 1500 & one\_fo & LL & 2.45$\pm$0.18 & 0.670$\pm$0.030 &             - &             - &              - &  2.89 \\
N~4013 &  144 & one\_fo & LL &  10.0$\pm$1.0 &   0.74$\pm$0.04 &             - &             - &              - &  1.41 \\
N~4013 & 1500 & one\_fo & UL & 3.41$\pm$0.22 & 0.578$\pm$0.020 &             - &             - &              - &  1.11 \\
N~4013 &  144 & one\_fo & UL &   8.8$\pm$0.8 &   1.05$\pm$0.05 &             - &             - &              - &  5.63 \\
N~4157 & 1500 & one\_fo & LR &   3.2$\pm$0.4 &   1.32$\pm$0.07 &             - &             - &              - &  0.68 \\
N~4157 &  144 &     one & LR &  15.7$\pm$2.3 &   1.25$\pm$0.07 &             - &             - &  0.55$\pm$0.26 &  5.26 \\
N~4157 & 1500 & one\_fo & UR &   3.7$\pm$0.6 &   0.96$\pm$0.06 &             - &             - &              - &  0.17 \\
N~4157 &  144 & one\_fo & UR &   6.9$\pm$1.2 &   2.31$\pm$0.19 &             - &             - &              - &  6.10 \\
N~4157 & 1500 & one\_fo & LM &  13.6$\pm$0.6 & 1.121$\pm$0.021 &             - &             - &              - &  4.79 \\
N~4157 &  144 & two\_fo & LM &      66$\pm$7 &   0.88$\pm$0.11 &   8.6$\pm$2.0 &   3.5$\pm$0.3 &              - &  2.34 \\
N~4157 & 1500 & two\_fo & UM &       8$\pm$7 &     0.7$\pm$0.4 &       9$\pm$8 & 1.25$\pm$0.20 &              - &  0.65 \\
N~4157 &  144 &     two & UM &      64$\pm$5 &   1.21$\pm$0.10 &   1.3$\pm$0.6 &      10$\pm$5 &  0.24$\pm$0.17 &  2.88 \\
N~4157 & 1500 & one\_fo & LL &   2.6$\pm$0.4 &   0.96$\pm$0.08 &             - &             - &              - &  0.03 \\
N~4157 &  144 & one\_fo & LL &   5.0$\pm$0.8 &   2.63$\pm$0.19 &             - &             - &              - &  4.17 \\
N~4157 & 1500 & one\_fo & UL &   2.4$\pm$0.3 &   1.45$\pm$0.07 &             - &             - &              - &  2.24 \\
N~4157 &  144 & one\_fo & UL &  10.0$\pm$1.1 &   2.59$\pm$0.13 &             - &             - &              - &  0.40 \\
N~4631 & 1500 & one\_fo & LR &   6.8$\pm$0.4 & 1.053$\pm$0.029 &             - &             - &              - &  1.11 \\
N~4631 &  144 & one\_fo & LR &  19.4$\pm$1.1 &   1.89$\pm$0.05 &             - &             - &              - &  0.74 \\
N~4631 & 1500 &     two & UR &  10.5$\pm$2.8 &   0.52$\pm$0.16 & 0.89$\pm$0.22 &   2.6$\pm$0.3 &   -0.6$\pm$0.4 &  0.39 \\
N~4631 &  144 & two\_fo & UR &  11.6$\pm$1.3 &   1.44$\pm$0.27 &   2.7$\pm$1.2 &   4.5$\pm$0.8 &              - &  1.07 \\
N~4631 & 1500 &     two & LM &     42$\pm$16 &   0.59$\pm$0.10 &   6.3$\pm$1.2 & 1.80$\pm$0.07 &   -0.7$\pm$0.4 &  1.88 \\
N~4631 &  144 & two\_fo & LM &  37.0$\pm$2.9 &   1.46$\pm$0.12 &   3.0$\pm$1.0 &   5.3$\pm$0.7 &              - &  5.03 \\
N~4631 & 1500 &     two & UM &     45$\pm$10 &   0.39$\pm$0.11 &   5.0$\pm$0.6 & 2.01$\pm$0.05 & -0.44$\pm$0.27 &  1.68 \\
N~4631 &  144 & one\_fo & UM &  19.1$\pm$0.8 &   2.90$\pm$0.05 &             - &             - &              - &  4.45 \\
N~4631 & 1500 & one\_fo & LL & 2.00$\pm$0.14 &   1.93$\pm$0.06 &             - &             - &              - &  1.12 \\
N~4631 &  144 & one\_fo & LL &   8.6$\pm$0.5 &   2.84$\pm$0.07 &             - &             - &              - &  0.86 \\
N~4631 & 1500 & one\_fo & UL & 1.15$\pm$0.09 &   2.15$\pm$0.09 &             - &             - &              - &  1.07 \\
N~4631 &  144 & one\_fo & UL &   6.1$\pm$0.3 &   3.71$\pm$0.10 &             - &             - &              - &  0.75 \\
 N~891 & 1500 & one\_fo & LR &   4.3$\pm$0.3 &   1.09$\pm$0.04 &             - &             - &              - &  2.55 \\
 N~891 &  144 & one\_fo & LR &  15.2$\pm$1.0 &   1.85$\pm$0.04 &             - &             - &              - &  4.02 \\
 N~891 & 1500 & one\_fo & UR &   4.5$\pm$0.3 &   1.35$\pm$0.04 &             - &             - &              - &  3.50 \\
 N~891 &  144 & two\_fo & UR &      32$\pm$5 &   0.77$\pm$0.15 &   6.7$\pm$1.4 & 3.04$\pm$0.26 &              - &  3.41 \\
 N~891 & 1500 & one\_fo & LM &  17.2$\pm$0.8 & 0.822$\pm$0.016 &             - &             - &              - &  7.41 \\
 N~891 &  144 &     two & LM &   188$\pm$113 &   0.87$\pm$0.08 &   5.8$\pm$2.1 &   2.9$\pm$0.4 &   -1.0$\pm$0.7 &  1.01 \\
 N~891 & 1500 & one\_fo & UM &  16.9$\pm$0.6 & 1.176$\pm$0.014 &             - &             - &              - &  5.88 \\
 N~891 &  144 &     two & UM &    111$\pm$18 &   1.05$\pm$0.10 &   6.6$\pm$2.3 &   3.6$\pm$0.5 & -0.33$\pm$0.27 &  0.50 \\
 N~891 & 1500 & one\_fo & LL &   7.4$\pm$0.6 &   1.05$\pm$0.03 &             - &             - &              - &  1.21 \\
 N~891 &  144 & two\_fo & LL &     43$\pm$22 &   0.37$\pm$0.21 &  13.9$\pm$1.6 & 2.18$\pm$0.08 &              - &  1.22 \\
 N~891 & 1500 & one\_fo & UL &   6.9$\pm$0.6 &   1.07$\pm$0.04 &             - &             - &              - &  1.05 \\
 N~891 &  144 & one\_fo & UL &  25.4$\pm$1.9 &   1.67$\pm$0.05 &             - &             - &              - &  1.05 \\
\bottomrule
\end{tabular}
\endgroup

==> CHANG-ES CR Transport MStein/tab_galaxy_param.tex <==
\begin{sidewaystable*}
\centering
\caption{Compostion of fundamental paramaters of all galxies in the sample of this work}
\label{tab:galaxy_param}
\begin{tabular}{lllrrlrrrrllrlrr}
\toprule
     Name &   R.A.(J2000) &  Decl.(J2000) &     i &   d25 &  Type &     d &   B-V &    MTF & v\textsubscript{rot} & M\textsubscript{*} &       $\alpha$ &   SFR & SFR\textsubscript{$\sigma$} & r\textsubscript{d25} & m\textsubscript{tot} \\
\midrule
  NGC~891 &  02h22m33.s41 &  +42d20m56.s9 &  84.0 &  12.2 &    Sb &   9.1 &  0.70 &   8.63 &                212.1 &      4.13$\pm$0.06 &  0.95$\pm$0.03 &  1.55 &               3.13$\pm$0.02 &                16.15 &                11.23 \\
 NGC~ 2683 &  08h52m41.s35 &  +33d25m18.s5 &  79.0 &   9.1 &    Sb &   6.3 &  0.75 &   7.35 &                202.6 &      1.49$\pm$0.02 &  0.89$\pm$0.08 &  0.09 &               1.34$\pm$0.02 &                 8.34 &                10.90 \\
 NGC~2820 &  09h21m45.s58 &  +64d15m28.s6 &  90.0 &   4.1 &   SBc &  26.5 &  0.23 &   3.41 &                162.8 &      0.47$\pm$0.01 &  0.88$\pm$0.02 &  0.62 &                4.2$\pm$0.02 &                15.80 &                10.99 \\
 NGC~3003 &  09h48m36.s05 &  +33d25m17.s4 &  90.0 &   6.0 &   Sbc &  25.4 &  0.28 &   1.19 &                120.6 &      0.48$\pm$0.01 &  0.88$\pm$0.04 &  0.67 &               1.11$\pm$0.02 &                22.17 &                10.88 \\
 NGC~3079 &  10h01m57.s80 &  +55d40m47.s3 &  88.0 &   7.7 &  SBcd &  20.6 &  0.53 &   8.11 &                208.4 &      4.73$\pm$0.07 &   0.6$\pm$0.02 &  3.46 &               6.54$\pm$0.02 &                23.07 &                11.37 \\
 NGC~3432 &  10h52m31.s13 &  +36d37m07.s6 &  82.0 &   4.9 &   SBm &   9.4 &  0.29 &   0.86 &                109.9 &        0.1$\pm$0.0 &  0.86$\pm$0.02 &  0.15 &               1.97$\pm$0.02 &                 6.70 &                10.28 \\
 NGC~ 3448 &  10h54m39.s24 &  +54d18m18.s8 &  78.0 &   4.9 &  S0-a &  24.5 &  0.31 &   1.15 &                119.5 &      0.56$\pm$0.01 &   0.6$\pm$0.02 &  0.92 &               7.55$\pm$0.02 &                17.46 &                10.76 \\
 NGC~ 3556 &  11h11m30.s97 &  +55d40m26.s8 &  81.0 &   7.8 &   SBc &  14.1 &  0.57 &   2.76 &                153.2 &      2.81$\pm$0.04 &  0.97$\pm$0.05 &  2.17 &               4.44$\pm$0.02 &                16.00 &                10.94 \\
 NGC~ 3877 &  11h46m07.s80 &  +47d29m41.s2 &  85.0 &   5.1 &    Sc &  17.7 &  0.65 &   2.87 &                155.1 &      2.74$\pm$0.04 &  0.89$\pm$0.02 &  0.92 &               3.43$\pm$0.02 &                13.13 &                10.87 \\
 NGC~ 4013 &  11h58m31.s38 &  +43d56m47.s7 &  84.0 &   4.7 &    Sb &  16.0 &  0.83 &   4.99 &                181.4 &      3.23$\pm$0.05 &  0.82$\pm$0.02 &  0.48 &               2.35$\pm$0.02 &                10.94 &                10.92 \\
 NGC~ 4096 &  12h06m01.s13 &  +47d28m42.s4 &  82.0 &   6.4 &  SABc &  10.3 &  0.50 &   2.26 &                144.8 &      0.61$\pm$0.01 &  0.94$\pm$0.02 &  0.27 &               2.46$\pm$0.02 &                 9.59 &                10.67 \\
 NGC~ 4157 &  12h11m04.s37 &  +50d29m04.s8 &  90.0 &   7.0 &  SABb &  15.6 &  0.64 &   5.75 &                188.9 &      2.92$\pm$0.04 &   0.9$\pm$0.02 &  1.25 &               5.77$\pm$0.02 &                15.88 &                11.12 \\
 NGC~ 4217 &  12h15m50.s90 &  +47d05m30.s4 &  78.0 &   5.1 &    Sb &  20.6 &  0.75 &   5.62 &                187.6 &      4.74$\pm$0.07 &  0.86$\pm$0.02 &  1.53 &               3.57$\pm$0.02 &                15.28 &                11.10 \\
 NGC~ 4244 &  12h17m29.s66 &  +37d48m25.s6 &  90.0 &  15.8 &    Sc &   4.4 &  0.41 &   0.57 &                 97.8 &       0.09$\pm$0.0 &  0.52$\pm$0.06 &  0.02 &               0.14$\pm$0.03 &                10.11 &                10.35 \\
 NGC~ 4565 &  12h36m20.s78 &  +25d59m15.s6 &  90.0 &  16.2 &   Sbc &  11.9 &  0.68 &  14.18 &                244.3 &      6.04$\pm$0.08 &  0.96$\pm$0.02 &  0.74 &               0.73$\pm$0.02 &                28.04 &                11.59 \\
 NGC~ 4631 &  12h42m08.s01 &  +32d32m29.s4 &  85.0 &  14.7 &  SBcd &   7.4 &  0.39 &   1.93 &                138.4 &      0.96$\pm$0.02 &   1.0$\pm$0.03 &  1.33 &                3.1$\pm$0.02 &                15.82 &                10.85 \\
 NGC~ 5297 &  13h46m23.s68 &  +43d52m20.s5 &  89.0 &   5.3 &  SABc &  40.4 &  0.50 &   5.81 &                189.5 &      3.69$\pm$0.07 &  0.96$\pm$0.05 &  1.27 &               2.41$\pm$0.02 &                31.14 &                11.42 \\
 NGC~ 5775 &  14h53m58.s00 &  +03d32m40.s1 &  84.0 &   3.9 &   Sbc &  28.9 &  0.66 &   5.57 &                187.2 &       7.72$\pm$0.1 &  0.92$\pm$0.02 &  5.28 &               6.58$\pm$0.02 &                16.39 &                11.13 \\
 NGC~ 5907 &  15h15m53.s77 &  +56d19m43.s6 &  90.0 &  11.2 &    Sc &  16.8 &  0.62 &  10.89 &                226.6 &      5.82$\pm$0.09 &  0.94$\pm$0.02 &  1.56 &               1.54$\pm$0.02 &                27.37 &                11.52 \\
\bottomrule
\end{tabular}
\end{sidewaystable*}


==> CHANG-ES CR Transport MStein/tab_obs_info.tex <==
\begin{table*}
\caption{Basic information about the galaxies EVLA C-Array observations.}
\label{tab:obs_info}
\centering
\begin{tabular}{l r r  r r r}% centered columns (4 columns)
    \hline
    \hline                        % inserts single horizontal line
    Galaxy  & Observing Date & Integration Time & Flux Cal. & Phase Cal. & SB ID \\
            & [M-D-Y]       & [M:S]             &   &\\
    \hline
    NGC~891  & 02-11-2012, 04-01-2012    & 46:40 & 3C48  & J0314+4314 & 8237609, 8182311\\
    NGC~3432 & 03-25-2012                & 43:20 & 3C286 & J1006+3454 & 8256114\\
    NGC~4013 & 03-31-2012                & 44:00 & 3C286 & J1219+4829 & 8318174\\
    NGC~4157 & 03-31-2012                & 41:00 & 3C286 & J1219+4829 & 8318174\\
    NGC~4631 & 02-04-2012                & 77:00 & 3C286 & J1221+2813 & 8312467\\

\hline                                   %inserts single line
\end{tabular}

\end{table*}

==> CHANG-ES CR Transport MStein/tab_radio_param.tex <==

\begin{table*}
	\caption{Flux densities and map properties of the analysed sample. We list the integrated flux density measurements in HBA (S\textsubscript{HBA} and L-Band (S\textsubscript{L-Band}), based on the described aperture, accounting for background noise ($\sigma$\textsubscript{HBA} \& $\sigma$\textsubscript{L-Band}) as well as calibration errors. Physical diameters, based on the $3\sigma$-contours in HBA, parallel  ($d_{\mathrm{HBA}}^{\mathrm{disk}}$) and orthogonal  ($d_{\mathrm{HBA}}^{\mathrm{halo}}$) to the galactic disk are also listed.
	}
	\label{tab:flux}
\centering          
\begin{tabular}{l l r r r r r r}     % 7 columns 
\hline\hline       
Galaxy & Ellipse $ a \times b$\tablefootmark{a} & $S$\textsubscript{HBA} & $\sigma$\textsubscript{HBA}\, & $S$\textsubscript{L-Band} & $\sigma$\textsubscript{Lband}& $d_{\mathrm{HBA}}^{\mathrm{disk}}$ & $d_{\mathrm{HBA}}^{\mathrm{halo}}$\\
& [arcmin$^2$] & [Jy] & [\muJyBeam] & [Jy] & [\muJyBeam] & [kpc] & [kpc]\\
\hline 

%  gal       ellipse            
NGC~891  &$5.9\times 4.55 $ &3.3$\pm$0.3 &207 &0.68$\pm$0.03 &31 & 28.4 & 15.6\\
NGC~3432 &$4.35\times 2.2 $ &0.30$\pm$0.03 &165 &0.086$\pm$0.004 &22 & 14.4 & 8.5\\
NGC~4013 &$2.36\times 1.45$ &0.151$\pm$0.015 &167 &0.0381$\pm$0.0019 &34 & 16.1 & 5.4\\
NGC~4157 &$4.25\times 2.08$ &1.01$\pm$0.10 &196 &0.180$\pm$0.009 &35 & 34.8 & 21.7 \\
NGC~4631 &$8.8 \times 7.5$ &4.46$\pm$0.45 &235& 1.03$\pm$0.05 &25  & 30.0 & 24.6\\
\hline                  
\end{tabular}
\tablefoot{
\tablefoottext{a}{Ellipses are defined in \citet{2022arXiv220400635H} and encompass the $3\sigma$-contours of the re-calibrated LoTSS map.}
}
\end{table*}



==> CHANG-ES CR Transport MStein/tab_scale_summary.tex <==
\begingroup
\renewcommand*{\arraystretch}{1.2}
\begin{table}
\centering
\caption{Fitted radio scale heights per galaxy. One and two component model are listed separately. For the two component models, we distinguish disk and halo scale heights. The Number of stripes (N) that have been fitted with each model is also indicated. If only one stripe has been fitted with a certain model, the uncertainty of the scale heights is computed within $\chi^2$-minimisation. If multiple stripes have been been fitted with a model, the uncertainty is computed via the standard deviation of the sample. }             % title of Table
\label{tab:scale_summary}      % is used to refer this table in the text
%\centering                          % used for centering table
\begin{tabular}{l r r r| r r}        % centered columns (4 columns)
    \hline\hline                 % inserts double horizontal lines
    Band  & \multicolumn{3}{c}{Two-Component} & \multicolumn{2}{|c}{One-Component} \\
            & Disk & Halo & N  & Overall & N \\
            &[kpc] &[kpc] &     &[kpc]\\% table heading \\
    \hline
    \multicolumn{4}{l|}{\textbf{NGC~891}}   \\
    L-Band  & -             &           - & 0 & 1.09$\pm$0.16 & 6 \\
    HBA     & 0.76$\pm$0.25 & 2.9$\pm$0.5 & 4 & 1.76$\pm$0.09 & 2    \\
    \hline
    \multicolumn{4}{l|}{\textbf{NGC~3432}}  \\
    L-Band  & - & - & 0 & 0.86$\pm$0.21 & 6   \\
    HBA     & - & - & 0 & 0.7$\pm$0.4 & 6    \\
    \hline
    \multicolumn{4}{l|}{\textbf{NGC~4013}} \\
    L-Band  & - & - & 0 & 0.60$\pm$0.08 & 6    \\
    HBA     & - & - & 0 & 0.75$\pm$0.14 & 6\\
    \hline
    \multicolumn{4}{l|}{\textbf{NGC~4157}}  \\
    L-Band  & 0.7$\pm$0.4 & 1.2$\pm$0.2 & 1 & 1.16$\pm$0.19 & 5  \\
    HBA     & 1.05$\pm$0.16 & 7$\pm$3 & 2 & 2.2$\pm$0.6 & 4\\
    \hline
    \multicolumn{4}{l|}{\textbf{NGC~4631}}  \\
    L-Band  & 0.50$\pm$0.08 & 2.1$\pm$0.3 & 3 & 1.7$\pm$0.5 & 3    \\
    HBA     & 1.45$\pm$0.01 & 4.9$\pm$0.4 & 2 & 2.8$\pm$0.6 & 4    \\
\hline                                   %inserts single line
\end{tabular}\\
\end{table}
\endgroup

==> CHANG-ES CR Transport MStein/tab_spin_param.tex <==
\centering
\begingroup
\renewcommand{\arraystretch}{1.3} % Default value: 1
\begin{tabular}{l l r r r r r r r}        % centered columns (4 columns)
    \hline\hline                 % inserts double horizontal lines
    Stripe & $z_{\mathrm{max}}$ & $\gamma$ & $\varv_c$ & $z_0$ & $\beta$ & z\textsubscript{c} & $\chi^2_\nu$\\ 
        &       [kpc]            &                                      & [km\,s\textsuperscript{-1}] & [kpc] &  & [kpc] & \\ % table heading 
    \hline                        % inserts single horizontal line
    \multicolumn{8}{c}{NGC~891}\\
    \hline
    LR  & 5.2      & 2.40$^{+0.08}_{-0.06}$ & 128$^{+18}_{-8}$ & 3.9$^{+0.5}_{-0.7}$ & 1.53$^{+0.04}_{-0.1}$ & 1.0$^{+0.6}_{-0.6}$ & 3.1	\\
    LM     & 5.2      & 2.16$^{+0.07}_{-0.05}$ & 152$^{+24}_{-11}$ & 2.4$^{+0.2}_{-0.3}$ & 1.73$^{+0.05}_{-0.08}$ & 0.2$^{+0.1}_{-0.1}$ & 3.4\\
    LL   & 5.2    & 2.20$^{+0.08}_{-0.07}$ & 129$^{+8}_{-6}$ & 4.9$^{+0.6}_{-0.6}$ & 1.85$^{+0.02}_{-0.05}$ & 2.3$^{+0.9}_{-0.7}$ & 3.6\\
    UR  & 6.0   & 2.32$^{+0.13}_{-0.07}$ & 167$^{+38}_{-14}$ & 5$^{+0.7}_{-0.9}$ & 1.79$^{+0.13}_{-0.18}$ & 1.1$^{+0.6}_{-0.6}$ & 2.2\\
    UM     & 7.8                         & 2.11$^{+0.08}_{-0.05}$ & 189$^{+26}_{-16}$ & 3.55$^{+0.3}_{-0.4}$ & 1.78$^{+0.06}_{-0.07}$ & 0.34$^{+0.12}_{-0.13}$ & 3.4\\ 
    UL   & 6.0   & 2.27$^{+0.08}_{-0.08}$ & 137$^{+9}_{-8}$ & 5.0$^{+0.8}_{-0.5}$ & 1.85$^{+0.03}_{-0.04}$ & 2.0$^{+0.9}_{-0.5}$ & 3.6\\
    \hline
    \multicolumn{8}{c}{NGC~3432}\\
    \hline
    LM & 3.9 & 2.13$^{+0.09}_{-0.16}$ & 240$^{+420}_{-135}$ & 3.0$^{+0.4}_{-0.2}$ & 2.10$^{+0.30}_{-0.35}$ & <0.9 & 1.5\\
    UM & 3.8 & 2.17$^{+0.12}_{-0.12}$ & 233$^{+760}_{-100}$ & 2.7$^{+0.2}_{-0.4}$ & 2.2$^{+0.20}_{-0.4}$ & <0.9 & 0.55	\\			\hline
    \multicolumn{8}{c}{NGC~4013}\\
    \hline
    LR & 3.6 & 2.4$^{+0.2}_{-0.2}$ & 122$^{+85}_{-26}$ & 2.5$^{+0.4}_{-0.3}$ & 2.0 & 0.9$^{+0.9}_{-0.6}$ & 0.4\\	
    LM & 2.9 & 2.30$^{+0.08}_{-0.04}$ & 100$^{+55}_{-14}$ & 1.1$^{+0.1}_{-0.1}$ & 1.6 & <1.4 & 1.7\\
    LL & 3.6 & 2.25$^{+0.15}_{-0.10}$ & 180$^{+610}_{-60}$ & 2.1$^{+0.4}_{-0.3}$ & 2.0 & <1.4 & 1	\\							
    \hline
    \multicolumn{8}{c}{NGC~4157}\\
    \hline
    %LR  & \textbf{No Fit} \\
    LM     & 7.2   & 2.21$^{+0.09}_{-0.06}$ & 177$^{+24}_{-12}$ & 4.7$^{+0.4}_{-0.7}$ & 1.72$^{+0.04}_{-0.10}$ & 0.4$^{+0.1}_{-0.2}$ & 1.7										 \\
    LL   & 6.0    & 2.39$^{+0.09}_{-0.10}$ & 128$^{+6}_{-5}$ & 8.2$^{+0.8}_{-1.1}$ & 2.21$^{+0.02}_{-0.02}$ & 4.7$^{+1.0}_{-1.2}$ & 0.5										\\
    %UR  & \textbf{No Fit}\\
    UM     & 7.1   & 2.26$^{+0.08}_{-0.08}$ & 226$^{+26}_{-24}$ & 5.3$^{+0.4}_{-0.5}$ & 2.05$^{+0.14}_{-0.12}$ & 0.6$^{+0.2}_{-0.2}$ & 2.81										\\
    UL   & 4.7  & 2.34$^{+0.10}_{-0.08}$ & 164$^{+10}_{-8}$ & 13.0$^{+2.0}_{-2.5}$ & 2.66$^{+0.02}_{-0.04}$ & 7.0$^{+0.5}_{-2.0}$ & 2.9																				\\
    \hline
    \multicolumn{8}{c}{NGC~4631}\\
    \hline
    LR  & 6.0    & 2.2$^{+0.16}_{-0.20}$ & 95$^{+12}_{-12}$ & 7.3$^{+1.7}_{-2.1}$ & 1.80$^{+0.10}_{-0.14}$ & 3.1$^{+3.2}_{-2.0}$ & 0.58																			\\
    LM     & 5.3     & 2.1$^{+0.10}_{-0.04}$ & 95$^{+20}_{-10}$ & 3.1$^{+0.5}_{-0.7}$ & 1.20$^{+0.08}_{-0.08}$ & <0.72 & 1.0																				\\
    LL   & 6.0    & 2.3$^{+0.30}_{-0.26}$ & 150$^{+55}_{-26}$ & 13$^{+7}_{-4}$ & 2.80$^{+0.10}_{-1.30}$ & 4.9$^{+0.9}_{-4.3}$ & 0.33																				\\
    UR  & 7.9   & 2.45$^{+0.24}_{-0.09}$ & 115$^{+114}_{-22}$ & 4.7$^{+1.0}_{-2.3}$ & 1.30$^{+0.15}_{-0.36}$ & <0.72 & 1.9																				\\
    UM     & 10.5     & 2.20$^{+0.14}_{-0.05}$ & 145$^{+34}_{-15}$ & 3.7$^{+0.4}_{-1.0}$ & 1.25$^{+0.10}_{-0.10}$ & <0.72 & 3.0																				\\
    UL   & 10.1     &2.45$^{+0.28}_{-0.12}$ & 125$^{+40}_{-15}$ & 9.4$^{+3.2}_{-3.1}$ & 1.25$^{+0.12}_{-0.14}$ & 0.5$^{+3.2}_{-0.5}$ & 0.5																				\\
\hline                                   %inserts single line
\end{tabular}

\endgroup

==> CHANG-ES CR Transport MStein/tab_thermal_emission.tex <==
\begin{table}
	\caption{Integrated thermal flux densities and non-thermal fractions in the analysed sample.}
	\label{tab:therm flux}
\centering          
\begin{tabular}{l r r r r}     % 7 columns 
\hline\hline       
Galaxy & $S_\mathrm{{HBA}^{th}}$ & $S_\mathrm{{L-Band}^{th}}$ & NTF\textsubscript{HBA} & NTF\textsubscript{L-Band}\\
& [Jy] & [Jy] & & \\
\hline 

%  gal       ellipse            
NGC~891  &0.056 &0.044 &0.98 &0.94 \\
NGC~3432 &0.013 &0.010 &0.95 &0.86 \\
NGC~4013 &0.006 &0.005 &0.96 &0.86 \\
NGC~4157 &0.018 &0.014 &0.98 &0.93 \\
NGC~4631 &0.117 &0.092 &0.97 &0.91 \\
\hline                  
\end{tabular}

\end{table}

==> CHANG-ES CR Transport MStein/total_int_figs.tex <==
\begin{figure*}
\centering

\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC891_CHANG-ES_L-Band.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC891_LOFAR_144_MHz.png}
\end{subfigure}
\\
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC3432_CHANG-ES_L-Band.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC3432_LOFAR_144_MHz.png}
\end{subfigure}
\\
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4013_CHANG-ES_L-Band.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4013_LOFAR_144_MHz.png}
\end{subfigure}
\caption{Total Intensity maps + contours from CHANG-ES L-band (left column) and LOFAR HBA (right column) after subtracting/masking point sources in the vicinity of the galaxy for NGC~891 (top row), NGC~3432 (middle row), and NGC~4013 (bottom row). Contours start at 3$\sigma$ above the background noise with an increment of 2. The beam is displayed in the bottom right corner of each map as a dark red circle.}
\label{fig:int_maps_1}
\end{figure*}

\begin{figure*}
\centering

\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4157_CHANG-ES_L-Band.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4157_LOFAR_144_MHz.png}
\end{subfigure}
\\
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4631_CHANG-ES_L-Band.png}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\includegraphics[width=1\linewidth]{figures/total_intensity/NGC4631_LOFAR_144_MHz.png}
\end{subfigure}
\caption{Continuation of Figure \ref{fig:int_maps_1}. Total Intensity maps from CHANG-ES L-band (left column) and LOFAR HBA (right column) after subtracting/masking point sources in the vicinity of the galaxy for NGC~4157 (top row), NGC~4631(bottom row).}
\label{fig:int_maps_2}
\end{figure*}

==> figures/total_intensity/tab_fit_params.tex <==
\begin{tabular}{lrlllllllr}
\toprule
N3432 & 1500 & one\_fo & LR & 0.32$\pm$0.04 &   1.16$\pm$0.09 &             - &             - &              - &  3.72 \\
N3432 &  144 & one\_fo & LR &   7.5$\pm$2.3 &   0.28$\pm$0.07 &             - &             - &              - &  2.41 \\
N3432 & 1500 &     one & UR & 2.20$\pm$0.20 &   0.45$\pm$0.03 &             - &             - &  0.54$\pm$0.07 &  4.27 \\
N3432 &  144 &     one & UR &     31$\pm$21 &   0.13$\pm$0.09 &             - &             - &  0.72$\pm$0.06 &  1.39 \\
N3432 & 1500 & one\_fo & LM & 4.68$\pm$0.27 & 0.940$\pm$0.028 &             - &             - &              - &  5.23 \\
N3432 &  144 & one\_fo & LM &  16.7$\pm$1.3 &   1.01$\pm$0.04 &             - &             - &              - &  1.11 \\
N3432 & 1500 & one\_fo & UM & 4.43$\pm$0.21 & 0.789$\pm$0.019 &             - &             - &              - & 10.07 \\
N3432 &  144 & one\_fo & UM &  16.7$\pm$1.2 &   0.87$\pm$0.03 &             - &             - &              - &  2.26 \\
N3432 & 1500 & one\_fo & LL & 2.47$\pm$0.29 &   0.91$\pm$0.05 &             - &             - &              - &  1.44 \\
N3432 &  144 & one\_fo & LL &   8.0$\pm$1.0 &   1.14$\pm$0.07 &             - &             - &              - &  1.77 \\
N3432 & 1500 & one\_fo & UL & 1.55$\pm$0.16 &   0.91$\pm$0.05 &             - &             - &              - &  1.97 \\
N3432 &  144 & one\_fo & UL &   6.2$\pm$0.8 &   1.03$\pm$0.07 &             - &             - &              - &  1.50 \\
N4013 & 1500 & one\_fo & LR & 2.09$\pm$0.19 & 0.607$\pm$0.026 &             - &             - &              - &  1.42 \\
N4013 &  144 & one\_fo & LR &   9.6$\pm$1.0 &   0.75$\pm$0.04 &             - &             - &              - &  0.55 \\
N4013 & 1500 & one\_fo & UR & 2.28$\pm$0.22 &   0.74$\pm$0.04 &             - &             - &              - &  0.96 \\
N4013 &  144 & one\_fo & UR &   9.1$\pm$1.0 &   0.87$\pm$0.04 &             - &             - &              - &  7.19 \\
N4013 & 1500 & one\_fo & LM &   4.3$\pm$0.4 & 0.549$\pm$0.025 &             - &             - &              - & 12.45 \\
N4013 &  144 & one\_fo & LM &  20.6$\pm$2.1 & 0.639$\pm$0.026 &             - &             - &              - &  3.15 \\
N4013 & 1500 & one\_fo & UM &   9.1$\pm$0.8 & 0.483$\pm$0.018 &             - &             - &              - &  3.54 \\
N4013 &  144 & one\_fo & UM &  30.9$\pm$2.8 & 0.642$\pm$0.022 &             - &             - &              - &  4.04 \\
N4013 & 1500 & one\_fo & LL & 2.45$\pm$0.18 & 0.670$\pm$0.030 &             - &             - &              - &  2.89 \\
N4013 &  144 & one\_fo & LL &  10.0$\pm$1.0 &   0.74$\pm$0.04 &             - &             - &              - &  1.41 \\
N4013 & 1500 & one\_fo & UL & 3.38$\pm$0.22 & 0.582$\pm$0.020 &             - &             - &              - &  2.52 \\
N4013 &  144 & two\_fo & UL &  12.8$\pm$1.7 &   0.64$\pm$0.13 &   0.6$\pm$0.6 &       5$\pm$5 &              - &  0.73 \\
N4157 & 1500 & one\_fo & LR &   3.2$\pm$0.4 &   1.32$\pm$0.07 &             - &             - &              - &  0.68 \\
N4157 &  144 &     one & LR &  15.7$\pm$2.3 &   1.25$\pm$0.07 &             - &             - &  0.55$\pm$0.26 &  5.26 \\
N4157 & 1500 & one\_fo & UR &   3.7$\pm$0.6 &   0.96$\pm$0.06 &             - &             - &              - &  0.17 \\
N4157 &  144 & one\_fo & UR &   6.9$\pm$1.2 &   2.31$\pm$0.19 &             - &             - &              - &  6.10 \\
N4157 & 1500 & one\_fo & LM &  13.6$\pm$0.6 & 1.121$\pm$0.021 &             - &             - &              - &  4.79 \\
N4157 &  144 & two\_fo & LM &      66$\pm$7 &   0.88$\pm$0.11 &   8.6$\pm$2.0 &   3.5$\pm$0.3 &              - &  2.34 \\
N4157 & 1500 & two\_fo & UM &       8$\pm$7 &     0.7$\pm$0.4 &       9$\pm$8 & 1.25$\pm$0.20 &              - &  0.65 \\
N4157 &  144 &     two & UM &      64$\pm$5 &   1.21$\pm$0.10 &   1.3$\pm$0.6 &      10$\pm$5 &  0.24$\pm$0.17 &  2.88 \\
N4157 & 1500 & one\_fo & LL &   2.6$\pm$0.4 &   0.96$\pm$0.08 &             - &             - &              - &  0.03 \\
N4157 &  144 & one\_fo & LL &   5.0$\pm$0.8 &   2.63$\pm$0.19 &             - &             - &              - &  4.17 \\
N4157 & 1500 & one\_fo & UL &   2.4$\pm$0.3 &   1.45$\pm$0.07 &             - &             - &              - &  2.24 \\
N4157 &  144 & one\_fo & UL &  10.0$\pm$1.1 &   2.59$\pm$0.13 &             - &             - &              - &  0.40 \\
N4631 & 1500 & one\_fo & LR &   6.8$\pm$0.4 & 1.053$\pm$0.029 &             - &             - &              - &  1.11 \\
N4631 &  144 & one\_fo & LR &  19.4$\pm$1.1 &   1.89$\pm$0.05 &             - &             - &              - &  0.74 \\
N4631 & 1500 &     two & UR &  10.5$\pm$2.8 &   0.52$\pm$0.16 & 0.89$\pm$0.22 &   2.6$\pm$0.3 &   -0.6$\pm$0.4 &  0.39 \\
N4631 &  144 & two\_fo & UR &  11.6$\pm$1.3 &   1.44$\pm$0.27 &   2.7$\pm$1.2 &   4.5$\pm$0.8 &              - &  1.07 \\
N4631 & 1500 &     two & LM &     42$\pm$16 &   0.59$\pm$0.10 &   6.3$\pm$1.2 & 1.80$\pm$0.07 &   -0.7$\pm$0.4 &  1.88 \\
N4631 &  144 & two\_fo & LM &  37.0$\pm$2.9 &   1.46$\pm$0.12 &   3.0$\pm$1.0 &   5.3$\pm$0.7 &              - &  5.03 \\
N4631 & 1500 &     two & UM &     45$\pm$10 &   0.39$\pm$0.11 &   5.0$\pm$0.6 & 2.01$\pm$0.05 & -0.44$\pm$0.27 &  1.68 \\
N4631 &  144 & one\_fo & UM &  19.1$\pm$0.8 &   2.90$\pm$0.05 &             - &             - &              - &  4.45 \\
N4631 & 1500 & one\_fo & LL & 2.00$\pm$0.14 &   1.93$\pm$0.06 &             - &             - &              - &  1.12 \\
N4631 &  144 & one\_fo & LL &   8.6$\pm$0.5 &   2.84$\pm$0.07 &             - &             - &              - &  0.86 \\
N4631 & 1500 & one\_fo & UL & 1.15$\pm$0.09 &   2.15$\pm$0.09 &             - &             - &              - &  1.07 \\
N4631 &  144 & one\_fo & UL &   6.1$\pm$0.3 &   3.71$\pm$0.10 &             - &             - &              - &  0.75 \\
 N891 & 1500 & one\_fo & LR &   4.3$\pm$0.3 &   1.09$\pm$0.04 &             - &             - &              - &  2.55 \\
 N891 &  144 & one\_fo & LR &  15.2$\pm$1.0 &   1.85$\pm$0.04 &             - &             - &              - &  4.02 \\
 N891 & 1500 & one\_fo & UR &   4.5$\pm$0.3 &   1.35$\pm$0.04 &             - &             - &              - &  3.50 \\
 N891 &  144 & two\_fo & UR &      32$\pm$5 &   0.77$\pm$0.15 &   6.7$\pm$1.4 & 3.04$\pm$0.26 &              - &  3.41 \\
 N891 & 1500 & one\_fo & LM &  17.2$\pm$0.8 & 0.822$\pm$0.016 &             - &             - &              - &  7.41 \\
 N891 &  144 &     two & LM &   188$\pm$113 &   0.87$\pm$0.08 &   5.8$\pm$2.1 &   2.9$\pm$0.4 &   -1.0$\pm$0.7 &  1.01 \\
 N891 & 1500 & one\_fo & UM &  16.9$\pm$0.6 & 1.176$\pm$0.014 &             - &             - &              - &  5.88 \\
 N891 &  144 &     two & UM &    111$\pm$18 &   1.05$\pm$0.10 &   6.6$\pm$2.3 &   3.6$\pm$0.5 & -0.33$\pm$0.27 &  0.50 \\
 N891 & 1500 & one\_fo & LL &   7.4$\pm$0.6 &   1.05$\pm$0.03 &             - &             - &              - &  1.21 \\
 N891 &  144 & two\_fo & LL &     43$\pm$22 &   0.37$\pm$0.21 &  13.9$\pm$1.6 & 2.18$\pm$0.08 &              - &  1.22 \\
 N891 & 1500 & one\_fo & UL &   6.9$\pm$0.6 &   1.07$\pm$0.04 &             - &             - &              - &  1.05 \\
 N891 &  144 & one\_fo & UL &  25.4$\pm$1.9 &   1.67$\pm$0.05 &             - &             - &              - &  1.05 \\
\bottomrule
\end{tabular}


==> tab_galaxy_param.tex <==
\begin{sidewaystable*}
\centering
\caption{Compostion of fundamental paramaters of all galxies in the sample of this work}
\label{tab:galaxy_param}
\begin{tabular}{lllrrlrrrrllrlrr}
\toprule
     Name &   R.A.(J2000) &  Decl.(J2000) &     i &   d25 &  Type &     d &   B-V &    MTF & v\textsubscript{rot} & M\textsubscript{*} &       $\alpha$ &   SFR & SFR\textsubscript{$\sigma$} & r\textsubscript{d25} & m\textsubscript{tot} \\
\midrule
  NGC~891 &  02h22m33.s41 &  +42d20m56.s9 &  84.0 &  12.2 &    Sb &   9.1 &  0.70 &   8.63 &                212.1 &      4.13$\pm$0.06 &  0.95$\pm$0.03 &  1.55 &               3.13$\pm$0.02 &                16.15 &                11.23 \\
 NGC~ 2683 &  08h52m41.s35 &  +33d25m18.s5 &  79.0 &   9.1 &    Sb &   6.3 &  0.75 &   7.35 &                202.6 &      1.49$\pm$0.02 &  0.89$\pm$0.08 &  0.09 &               1.34$\pm$0.02 &                 8.34 &                10.90 \\
 NGC~2820 &  09h21m45.s58 &  +64d15m28.s6 &  90.0 &   4.1 &   SBc &  26.5 &  0.23 &   3.41 &                162.8 &      0.47$\pm$0.01 &  0.88$\pm$0.02 &  0.62 &                4.2$\pm$0.02 &                15.80 &                10.99 \\
 NGC~3003 &  09h48m36.s05 &  +33d25m17.s4 &  90.0 &   6.0 &   Sbc &  25.4 &  0.28 &   1.19 &                120.6 &      0.48$\pm$0.01 &  0.88$\pm$0.04 &  0.67 &               1.11$\pm$0.02 &                22.17 &                10.88 \\
 NGC~3079 &  10h01m57.s80 &  +55d40m47.s3 &  88.0 &   7.7 &  SBcd &  20.6 &  0.53 &   8.11 &                208.4 &      4.73$\pm$0.07 &   0.6$\pm$0.02 &  3.46 &               6.54$\pm$0.02 &                23.07 &                11.37 \\
 NGC~3432 &  10h52m31.s13 &  +36d37m07.s6 &  82.0 &   4.9 &   SBm &   9.4 &  0.29 &   0.86 &                109.9 &        0.1$\pm$0.0 &  0.86$\pm$0.02 &  0.15 &               1.97$\pm$0.02 &                 6.70 &                10.28 \\
 NGC~ 3448 &  10h54m39.s24 &  +54d18m18.s8 &  78.0 &   4.9 &  S0-a &  24.5 &  0.31 &   1.15 &                119.5 &      0.56$\pm$0.01 &   0.6$\pm$0.02 &  0.92 &               7.55$\pm$0.02 &                17.46 &                10.76 \\
 NGC~ 3556 &  11h11m30.s97 &  +55d40m26.s8 &  81.0 &   7.8 &   SBc &  14.1 &  0.57 &   2.76 &                153.2 &      2.81$\pm$0.04 &  0.97$\pm$0.05 &  2.17 &               4.44$\pm$0.02 &                16.00 &                10.94 \\
 NGC~ 3877 &  11h46m07.s80 &  +47d29m41.s2 &  85.0 &   5.1 &    Sc &  17.7 &  0.65 &   2.87 &                155.1 &      2.74$\pm$0.04 &  0.89$\pm$0.02 &  0.92 &               3.43$\pm$0.02 &                13.13 &                10.87 \\
 NGC~ 4013 &  11h58m31.s38 &  +43d56m47.s7 &  84.0 &   4.7 &    Sb &  16.0 &  0.83 &   4.99 &                181.4 &      3.23$\pm$0.05 &  0.82$\pm$0.02 &  0.48 &               2.35$\pm$0.02 &                10.94 &                10.92 \\
 NGC~ 4096 &  12h06m01.s13 &  +47d28m42.s4 &  82.0 &   6.4 &  SABc &  10.3 &  0.50 &   2.26 &                144.8 &      0.61$\pm$0.01 &  0.94$\pm$0.02 &  0.27 &               2.46$\pm$0.02 &                 9.59 &                10.67 \\
 NGC~ 4157 &  12h11m04.s37 &  +50d29m04.s8 &  90.0 &   7.0 &  SABb &  15.6 &  0.64 &   5.75 &                188.9 &      2.92$\pm$0.04 &   0.9$\pm$0.02 &  1.25 &               5.77$\pm$0.02 &                15.88 &                11.12 \\
 NGC~ 4217 &  12h15m50.s90 &  +47d05m30.s4 &  78.0 &   5.1 &    Sb &  20.6 &  0.75 &   5.62 &                187.6 &      4.74$\pm$0.07 &  0.86$\pm$0.02 &  1.53 &               3.57$\pm$0.02 &                15.28 &                11.10 \\
 NGC~ 4244 &  12h17m29.s66 &  +37d48m25.s6 &  90.0 &  15.8 &    Sc &   4.4 &  0.41 &   0.57 &                 97.8 &       0.09$\pm$0.0 &  0.52$\pm$0.06 &  0.02 &               0.14$\pm$0.03 &                10.11 &                10.35 \\
 NGC~ 4565 &  12h36m20.s78 &  +25d59m15.s6 &  90.0 &  16.2 &   Sbc &  11.9 &  0.68 &  14.18 &                244.3 &      6.04$\pm$0.08 &  0.96$\pm$0.02 &  0.74 &               0.73$\pm$0.02 &                28.04 &                11.59 \\
 NGC~ 4631 &  12h42m08.s01 &  +32d32m29.s4 &  85.0 &  14.7 &  SBcd &   7.4 &  0.39 &   1.93 &                138.4 &      0.96$\pm$0.02 &   1.0$\pm$0.03 &  1.33 &                3.1$\pm$0.02 &                15.82 &                10.85 \\
 NGC~ 5297 &  13h46m23.s68 &  +43d52m20.s5 &  89.0 &   5.3 &  SABc &  40.4 &  0.50 &   5.81 &                189.5 &      3.69$\pm$0.07 &  0.96$\pm$0.05 &  1.27 &               2.41$\pm$0.02 &                31.14 &                11.42 \\
 NGC~ 5775 &  14h53m58.s00 &  +03d32m40.s1 &  84.0 &   3.9 &   Sbc &  28.9 &  0.66 &   5.57 &                187.2 &       7.72$\pm$0.1 &  0.92$\pm$0.02 &  5.28 &               6.58$\pm$0.02 &                16.39 &                11.13 \\
 NGC~ 5907 &  15h15m53.s77 &  +56d19m43.s6 &  90.0 &  11.2 &    Sc &  16.8 &  0.62 &  10.89 &                226.6 &      5.82$\pm$0.09 &  0.94$\pm$0.02 &  1.56 &               1.54$\pm$0.02 &                27.37 &                11.52 \\
\bottomrule
\end{tabular}
\end{sidewaystable*}

